ConSept: Continual Semantic Segmentation via Adapter-based Vision Transformer

In this paper, we delve into the realm of vision transformers for continual semantic segmentation, a problem that has not been sufficiently explored in previous literature. Empirical investigations on the adaptation of existing frameworks to vanilla ViT reveal that incorporating visual adapters into ViTs or fine-tuning ViTs with distillation terms is advantageous for enhancing the segmentation capability of novel classes. These findings motivate us to propose Continual semantic Segmentation via Adapter-based ViT, namely ConSept. Within the simplified architecture of ViT with linear segmentation head, ConSept integrates lightweight attention-based adapters into vanilla ViTs. Capitalizing on the feature adaptation abilities of these adapters, ConSept not only retains superior segmentation ability for old classes, but also attains promising segmentation quality for novel classes. To further harness the intrinsic anti-catastrophic forgetting ability of ConSept and concurrently enhance the segmentation capabilities for both old and new classes, we propose two key strategies: distillation with a deterministic old-classes boundary for improved anti-catastrophic forgetting, and dual dice losses to regularize segmentation maps, thereby improving overall segmentation performance. Extensive experiments show the effectiveness of ConSept on multiple continual semantic segmentation benchmarks under overlapped or disjoint settings. Code will be publicly available at \url{https://github.com/DongSky/ConSept}.

==> sections/introduction_old.tex <==
\section{Introduction}\label{sec:introduction}
% Leveraging self-attention mechanisms~\cite{vaswani2017attention} and feed-forward networks, 
% Vision Transformers (ViTs)~\cite{dosovitskiy2020image} have achieved remarkable progress on various visual recognition tasks~\cite{touvron2021training,Liu_2021_ICCV,li2022exploring,YOLOS,caron2021emerging,xie2021segformer,Kirillov2023segment,cheng2021mask2former}. 
% %
% Benefiting from better training objectives, stronger regularization, and complicated data augmentation, modern ViTs demonstrate promising performance on different learning paradigms, including fully-supervised learning~\cite{li2022exploring,strudel2021segmenter}, weakly- and semi-supervised learning~\cite{weng2022semi,cai2022semi,bai2022weakly,zhu2023weaktr}, and few-shot learning~\cite{dong2022self,kang2023distilling}. 
% %
% Notably, all mentioned works mainly focus on improving the generalization ability or performance on corresponding benchmarks.
% %
% However, corresponding training objectives are designed for target training data and distribution, but ignoring to maintain the generalization capability on old classes, thus resulting in catastrophic forgetting phenomenon~\cite{french1999catastrophic,li2016learning}. 
% %
% To tackle this issue, recent works have started early explorations on ViT-based continual learning~\cite{wang2022learning,wang2022dualprompt,smith2023coda,jeeveswaran2023birt,Mohamed_2023_CVPR}. 
% %
% In this paper, we focus on class-incremental setting~\cite{cermelli2020modeling,wang2022learning,wang2022dualprompt} to discuss ViT-based continual learning. 
Vision Transformers (ViTs)~\cite{dosovitskiy2020image} have achieved remarkable progress on various visual recognition tasks~\cite{touvron2021training,Liu_2021_ICCV,li2022exploring,YOLOS,caron2021emerging,xie2021segformer,Kirillov2023segment,cheng2021mask2former}. 
%
Such progress can be attributed to enhanced training objectives, robust regularization techniques, and sophisticated data augmentation strategies. 
%
Therefore, modern ViTs exhibit promising performance across various learning paradigms, encompassing fully-supervised learning~\cite{li2022exploring,strudel2021segmenter}, weakly- and semi-supervised learning~\cite{weng2022semi,cai2022semi,bai2022weakly,zhu2023weaktr}, as well as few-shot learning scenarios~\cite{dong2022self,kang2023distilling}.
%
It is noteworthy that the aforementioned studies primarily concentrate on improving generalization capabilities or achieving superior performance on specific benchmarks. 
%
\begin{figure}[t]
    % %%%\vspace{-0.5em}
    \begin{center}
    \includegraphics[width=0.48\textwidth]{figs/overview_page1.pdf}
    % \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}} 
    \end{center}
    \vspace{-1em}
    \caption{
        Performance comparison between previous state-of-the-art methods~\cite{cermelli2020modeling,zhang2022microseg,shang2023incrementer} and our ConSept. ConSept obtains better performance on all four PASCAL VOC benchmarks with \emph{overlapped} setting. Best viewed in color.
    }
    \vspace{-1em}
    \label{fig:overview_voc}
    \end{figure}
%
However, the formulated training objectives are tailored to the characteristics of the target training data and distribution, thereby neglecting the preservation of generalization capability for previously learned classes.
%
Consequently, this oversight gives rise to the phenomenon of catastrophic forgetting~\cite{french1999catastrophic,li2016learning}. 
%
To tackle this challenge, recent investigations have initiated early explorations into ViT-based continual learning~\cite{wang2022learning,wang2022dualprompt,smith2023coda,jeeveswaran2023birt,Mohamed_2023_CVPR}.
%
This paper specifically focuses on the class-incremental setting~\cite{cermelli2020modeling,wang2022learning,wang2022dualprompt} within the context of ViT-based continual learning.

% Compared to conventional continual image classification, continual semantic segmentation~\cite{cermelli2020modeling,michieli2019incremental,douillard2021plop} is much more challenging. 
% %
% This task needs to predict pixel-level labels rather than image-level prediction for given images with class-incremental setting. 
% %
% Conventional continual semantic segmentation approaches mainly focus on classical CNN feature extractors (\emph{e.g.}, ResNet-101~\cite{He2016DeepRL}) and complicated segmentation decoders (\emph{e.g.}, DeepLab V3~\cite{chen2017deeplab}) as baseline method, 
% %
% and introducing distillation methods~\cite{cermelli2020modeling,douillard2021plop,cha2021ssul} or regularization terms~\cite{michieli2021continual,lin2022continual} to improve the anti-catastrophic forgetting capability.
% %
% Since vanilla vision transformers have demonstrated remarkable performance on different image segmentation benchmarks~\cite{zhou2017scene,everingham2010pascal,lin2014microsoft}, 
% %
% this progress motivates us to investigate two following questions. 
% %
% First, starting from any CNN-based continual semantic segmentation framework~\cite{cermelli2020modeling,douillard2021plop,cha2021ssul}, 
% %
% could we simply replace the conventional CNN feature extractor~\cite{He2016DeepRL} by a pretrained vanilla ViT~\cite{dosovitskiy2020image,caron2021emerging,zhou2022mugs} to obtain better performance? 
% %
% And second, if not, how to formulate a effective continual segmentation framework via vision transformers with simple linear segmentation heads? 
In contrast to traditional continual image classification, the pursuit of continual semantic segmentation~\cite{cermelli2020modeling,michieli2019incremental,douillard2021plop} poses significantly greater challenges. 
%
This undertaking necessitates the prediction of pixel-level labels rather than image-level predictions in a class-incremental setting. 
%
Conventional methodologies for continual semantic segmentation primarily center around employing classical CNN feature extractors (\emph{e.g.}, ResNet-101~\cite{He2016DeepRL}) and intricate segmentation decoders (\emph{e.g.}, DeepLab V3~\cite{chen2017deeplab}) as baseline methods. 
%
These approaches introduce distillation methods~\cite{cermelli2020modeling,douillard2021plop,cha2021ssul} or regularization terms~\cite{michieli2021continual,lin2022continual} to enhance their anti-catastrophic forgetting capabilities.
%
Given the outstanding performance of vanilla vision transformers in diverse generic image segmentation benchmarks~\cite{zhou2017scene,everingham2010pascal,lin2014microsoft}, this progress motivates us to investigate two fundamental questions. 
%
Firstly, starting from any CNN-based continual semantic segmentation framework~\cite{cermelli2020modeling,douillard2021plop,cha2021ssul}, can we effectively substitute the conventional CNN feature extractor~\cite{He2016DeepRL} with a pretrained vanilla Vision Transformer (ViT)~\cite{dosovitskiy2020image,caron2021emerging,zhou2022mugs} to achieve improved performance? 
%
Secondly, if not, how can we formulate an effective continual segmentation framework using vision transformers with straightforward linear segmentation heads?



% For the first question, the answer is unfortunately negative. 
% %
% % Based on a specific continual semantic segmentation method, \emph{e.g.}, SSUL~\cite{cha2021ssul}, 
% % %
% % when simply replacing ImageNet-pretrained~\cite{deng2009imagenet} CNN feature extractor~\cite{He2016DeepRL} with vanilla ViT, 
% When adopting vanilla ViT to a classical CNN-based continual semantic segmentation method, \emph{e.g.}, SSUL~\cite{cha2021ssul}, 
% %
% the ViT-based continual segmenter achieves the similar performance on base classes, but suffers much lower mIoU on novel classes, thus resulting in lower overall performance. 
% %
% Based on empirical study regarding pretrained vision transformer, we conclude that: 
% %
% the frozen pretrained vision transformer tends to overfit on base classes, thus remaining feasible anti-catastrophic forgetting capability on base classes, 
% %
% but restricting the generalization ability to novel categories. 
% %
% % We conduct empirical analysis in Sec.~\ref{sec:pre_analysis} to explore the directions of tackling this issue. 
% % These results indicates that, 
% Meanwhile, further empirical analysis in Sec.~\ref{sec:pre_analysis} indicates that: 
% %
% both \textbf{1)} inserting adapters into ViT feature extractor, and \textbf{2)} additional distillation terms benefits to both old and novel classes for continual semantic segmentation. %can lead to better segmentation quality for novel classes, and without largely losing the significant segmentation capability on base classes. 
% %
% These results naturally motivate us to design an adapter-based vision transformer with specially designed continual learning frameworks, such that even without complex segmentation decoders, 
% %
% \textbf{1)} it improves the anti-catastrophic forgetting ability for base classes, meanwhile \textbf{2)} it obtains the robust segmentation ability on novel classes.
% %
% Based on these observations, we propose a simple yet effective continual semantic segmentation method namely ConSept. 
% %
% Keeping the simple macro architecture with only ViT~\cite{dosovitskiy2020image} and linear segmentation head, 
% %
% ConSept offers our insights for ViT-based continual semantic segmentation, which is illustrated as follows.
%, which can effectively improves the anti-catastrophic forgetting capability of base classes, 
%
% meanwhile leading to better segmentation quality for novel classes, thus achieving better overall segmentation ability. 

Regrettably, the answer to the first question is negative. 
%
Upon integrating a vanilla Vision Transformer (ViT) into a classical CNN-based continual semantic segmentation method (\emph{e.g.}, SSUL~\cite{cha2021ssul}), 
%
the ViT-based continual segmenter exhibits comparable performance on base classes but experiences a notable decline in mIoU on novel classes, consequently resulting in an overall performance degeneration. 
%
Through empirical investigation into pretrained vision transformers, it is discerned that a frozen pretrained vision transformer tends to exhibit overfitting tendencies on base classes, 
%
thereby preserving feasible anti-catastrophic forgetting capability on these classes while concurrently constraining its generalization capacity to novel categories. 
%
Furthermore, a comprehensive empirical analysis in Section~\ref{sec:pre_analysis} reveals that both \textbf{1)} incorporating adapters into the ViT feature extractor, 
%
and \textbf{2)} introducing additional distillation terms prove advantageous for both old and novel classes in the context of continual semantic segmentation.
%
These findings naturally motivate us to design an adapter-based vision transformer integrated with specifically designed continual learning frameworks. 
%
Such an architecture, even in the absence of complex segmentation decoders, accomplishes the dual objectives of: 
%
\textbf{1)} enhancing anti-catastrophic forgetting ability for base classes, 
%
and \textbf{2)} attaining robust segmentation capability for novel classes. 
%
Motivated by these observations, we present ConSept, a straightforward yet efficacious continual semantic segmentation method. 
%
Maintaining a simplistic macro architecture comprising solely ViT~\cite{dosovitskiy2020image} and a linear segmentation head, 
%
ConSept offers our insights into ViT-based continual semantic segmentation, which is illustrated as follows.

% For frozen ViT, the most significant issue is improving unpromising segmentation ability on novel categories. 
% %
% To tackle this issue, we propose \textbf{fine-tuning with adapters for better generalization}, which is the most significant component of ConSept. 
% %
% % Inspired by parameter-efficient fine-tuning~\cite{chen2022convadapter,nie2022protuning}, 
% Specifically, 
% %
% Inspired by previous visual adapters~\cite{nie2022protuning,chen2022convadapter,chen2023vision} for transfer learning, 
% %
% we insert a shallow convolution-based stem block as well as additional lightweight attention-based adapters into pretrained ViT~\cite{dosovitskiy2020image} and obtain a dual-path feature extractor. 
% %
% Then image features refined by adapters are fed into an extremely simple linear segmentation head for prediction.
% % ConSept also leverages a dual-path ViT adapter architecture~\cite{chen2023vision} into pretrained ViT backbone. 
% %
% With $<10\%$ more additional parameters, 
% %
% ConSept significantly improves the generalization ability for novel classes effectively and efficiently, 
% %
% especially does not further eliminate the anti-catastrophic forgetting capability for base classes. %This improvement is the most critical component of ConSept.
% %
% Besides, previous methods~\cite{cha2021ssul,zhang2022microseg} usually freeze the feature extractors during training for anti-catastrophic forgetting ability. 
% %
% However, for ViT-based scenarios, this strategy dramatically restricts the segmentation ability of novel classes. 
% %
% % Different from \cite{cha2021ssul,zhang2022microseg}, 
% To ease the side effect from frozen ViT and exploit the power of adapters in ConSept,
% %
% we fine-tune the whole feature extractor to ensure the network can learn representative features for new concepts, 
% %
% thus further ensuring the generalization ability on novel classes. 

A primary concern with the frozen Vision Transformer (ViT) lies in its suboptimal segmentation performance on novel categories. 
%
In response to this challenge, we propose a pivotal enhancement within ConSept namely \textbf{fine-tuning with adapters for better generalization}, which is the most significant component of ConSept. 
%
% This approach constitutes a fundamental component of ConSept, addressing the critical issue of refining the segmentation ability on novel categories. 
%
Drawing inspiration from prior work on visual adapters~\cite{nie2022protuning,chen2022convadapter,chen2023vision} for transfer learning, we integrate a shallow convolution-based stem block and lightweight attention-based adapters into the pretrained ViT~\cite{dosovitskiy2020image}, resulting in a dual-path feature extractor. 
%
The image features refined by these adapters are subsequently input into an exceedingly simple linear segmentation head for prediction. 
%
With $<10\%$ more additional parameters, ConSept notably enhances the generalization ability for novel classes, preserving the anti-catastrophic forgetting capability for base classes effectively and efficiently.
%
Notably, conventional approaches~\cite{cha2021ssul,zhang2022microseg} often adopt the strategy of freezing feature extractors during training to mitigate the risk of catastrophic forgetting. 
%
However, in the context of ViT-based scenarios shown in Table~\ref{table:pre_vanilla_vit}, this strategy imposes substantial limitations on the segmentation ability of novel classes. 
%
To mitigate the adverse effects associated with frozen ViT and leverage the benefits of adapters within ConSept, we advocate fine-tuning the entire feature extractor. 
%
This strategic adjustment ensures the network's capacity to learn representative features for new concepts, thereby reinforcing its generalization ability on novel classes.


% In addition to adapter-based macro design for ConSept, to further exploit the power of adapter-based ConSept for continual segmentation, 
% %
% we propose two more critical strategies for ConSept.
% %
% First is \textbf{distillation with deterministic old-classes boundary for better anti-catastrophic forgetting. }
% %
% Since naive fine-tuning ViT feature extractor without any constraints still lead to catastrophic forgetting for base classes~\cite{shang2023incrementer,cermelli2020modeling}.
% %
% To further enhance corresponding capability, 
% %
% we propose \textbf{1)} leveraging dense mean-square loss and dense contrastive loss to distill image features between old and new models, 
% %
% and \textbf{2)} freezing linear head for old classes to maintain the concrete decision boundary for segmentation. 
% %
% And second is \textbf{dual dice losses for better regularization. }
% %
% % To better discriminate old classes and novel classes, 
% Specifically, we leverage two dice loss terms to measure errors among segmentation predictions. 
% %
% For class-specific dice loss term, we follow the classical dice loss~\cite{sudre2017generalised} to improve overall segmentation ability. 
% %
% And for old-new dice loss term, we binarize the pseudo ground-truth maps to old classes region and new classes region, 
% %
% and apply dice loss constraint to improve segmentation quality for novel classes.

In conjunction with the adapter-based macro design implemented in ConSept, we introduce two additional pivotal strategies aimed at further harnessing the efficacy of adapter-based ConSept for continual segmentation. 
%
The first strategy involves \textbf{distillation with deterministic old-classes boundary for better anti-catastrophic forgetting}. 
%
Since naive fine-tuning ViT feature extractor without any constraints still lead to catastrophic forgetting for base classes~\cite{shang2023incrementer,cermelli2020modeling}. To further enhance the anti-forgetting capability, we propose: 
%
\begin{itemize}
    \item \textbf{1)} employing dense mean-square loss and dense contrastive loss to distill image features between old and new models.
    \item \textbf{2)} preserving the frozen state of the linear head for old classes to uphold a well-defined decision boundary for segmentation.
\end{itemize}
%
The second strategy revolves around \textbf{dual dice losses for better regularization}. 
%
Specifically, we incorporate two dice loss terms to assess errors in segmentation predictions. 
%
For the class-specific dice loss term, we adhere to the classical dice loss~\cite{sudre2017generalised} to enhance overall segmentation proficiency. 
%
Simultaneously, for the old-new dice loss term, we binarize the pseudo ground-truth maps into regions corresponding to old classes and new classes, and apply dice loss constraint to improve segmentation quality for novel classes.

Empirical experiments have been conducted on two challenging continual semantic segmentation benchmarks 
%
(\emph{i.e.}, PASCAL VOC~\cite{everingham2010pascal} and ADE20K~\cite{zhou2017scene}). 
%
As shown in Fig.~\ref{fig:overview_voc}, 
%
our ConSept achieves comparable performance on PASCAL VOC benchmarks under various class-incremental learning steps. 
%
Meanwhile, even in more challenging scenarios with much more classes, 
%
our ConSept can also obtain remarkable segmentation performance for both base and novel classes. 
%
Above promising quantitative and qualitative results demonstrate that, 
%
\emph{albeit without relying on extra object proposals from external models~\cite{zhang2022microseg,zhang2023coinseg} or heavy segmentation decoder~\cite{shang2023incrementer}}, 
%
ConSept still enhances the anti-catastrophic forgetting capability of base classes, 
%
meanwhile effectively improves the segmentation ability for novel classes. 
%
Moreover, our method provides a strong and stable baseline for ViT-based continual semantic segmentation tasks, 
%
and also inspire future research directions.
